From Pretraining Data to Language Models to Downstream Tasks: Tracking the Trails of Political Biases Leading to Unfair NLP Models

Language models (LMs) are pretrained on diverse data sources, including news, discussion forums, books, and online encyclopedias. A significant portion of this data includes opinions and perspectives which, on one hand, celebrate democracy and diversity of ideas, and on the other hand are inherently socially biased. Our work develops new methods to (1) measure political biases in LMs trained on such corpora, along social and economic axes, and (2) measure the fairness of downstream NLP models trained on top of politically biased LMs. We focus on hate speech and misinformation detection, aiming to empirically quantify the effects of political (social, economic) biases in pretraining data on the fairness of high-stakes social-oriented tasks. Our findings reveal that pretrained LMs do have political leanings that reinforce the polarization present in pretraining corpora, propagating social biases into hate speech predictions and misinformation detectors. We discuss the implications of our findings for NLP research and propose future directions to mitigate unfairness.

==> intro-backup.tex <==
\section{Introduction}


With the increasing popularity of social media, the volume of online political discussions has significantly grown in the past decade \citep{Valenzuela2012SocialNT, Enikolopov2019PoliticalEO, rainie2012social}. Social media has become a major source of political news dissemination \citep{kumpel2015news, hermida2012share, hermida2016social} with record-high user engagement in the online political discourse \citep{garimella2018political, mustafaraj2011edited, velasquez2012social}. This has led to societal problems such as politically-motivated hate speech and hyperpartisan misinformation that prey on communities with certain identities \citep{josey2010hate, sachdeva2022targeted} and ideological beliefs \citep{kucharski2016study, rhodes2022filter}, while humanity has made great strides to combat them with politically neutral and impartial actors \citep{chetty2018hate, kyriakidou2021journalistic, modha2020detecting}.

Since language is the primary medium of online political discourse, pretrained language models have been increasingly leveraged to promote online social good, such as automatically identifying hate speech \citep{ramponi-tonelli-2022-features, hartvigsen-etal-2022-toxigen} and online misinformation \citep{mehta-etal-2022-tackling, wu-etal-2022-cross}. Although pretrained language models have achieved relative success in these domains, it is generally assumed that language models, similar to their human counterparts such as PolitiFact \footnote{\url{https://www.politifact.com/}} and HateWatch \footnote{\url{https://www.splcenter.org/hatewatch}}, can serve as politically impartial judges who do not heavily favor one side or the other in the decision-making process \citep{chetty2018hate, kyriakidou2021journalistic}. However, it is not well understood to what extent language models are politically biased, which undermines the use of LM-based solutions for tasks such as hate speech and political misinformation detection. If pretrained LMs do have political biases, they might exhibit biased behavior in high-stakes downstream tasks, which could have negative consequences for a fair, informative, and non-discriminatory online environment \citep{jiang2020reasoning, binns2017like, gongane2022detection}.

In this work, we investigate the underlying political leanings of pretrained language models and their effect on downstream task behavior.

\textbf{RQ1: How can we measure the political leaning of pretrained language models?}
Grounded in the two-axis political spectrum theories \citep{eysenck1957sense, rokeach1973nature, gindler2021theory} and the political compass test\footnote{\url{https://www.politicalcompass.org/test}}, we collect 62 propositions that reflect the major debates regarding social and economic issues. We then curate prompts to probe the opinions of pretrained LMs towards these propositions and map their responses to the two-dimensional ideological space, as illustrated in Figure \ref{fig:teaser}. Armed with our proposed framework, we evaluate the political leaning of existing LM checkpoints as well as those further pretrained on more partisan corpora. Experiments demonstrate that different pretrained LMs \textit{do} have different underlying political leanings, while language models are capable of picking up the political polarization present in pretraining corpora.

\textbf{RQ2: How do the political biases of LMs affect their behavior in downstream tasks?} We focus on two tasks, hate speech detection and misinformation identification, for which many LM-based solutions have been proposed. Specifically, we investigate the behavior of four variations of RoBERTa \citep{Liu2019RoBERTaAR} that are pretrained on left- and right-leaning corpora from news and social media. Our experiments reveal that while the overall performance metrics remain close, these models exhibit significantly different behaviors when it comes to detecting hate speech against different identity groups and identifying misinformation from different sources. These results establish a link between political polarization in pretraining corpora and the fairness of LM-based solutions to downstream tasks with social bias implications.
